General-purpose Tagging of Freesound Audio with AudioSet Labels: Task Description, Dataset, and Baseline

This paper describes Task 2 of the DCASE 2018 Challenge, titled "General-purpose audio tagging of Freesound content with AudioSet labels". This task was hosted on the Kaggle platform as "Freesound General-Purpose Audio Tagging Challenge". The goal of the task is to build an audio tagging system that can recognize the category of an audio clip from a subset of 41 diverse categories drawn from the AudioSet Ontology. We present the task, the dataset prepared for the competition, and a baseline system.

==> S1_Intro.tex <==
The sounds in our everyday environment carry a huge amount of information including the context of our whereabouts and the events occurring nearby.
Humans are able to recognize and discern many fine details from environmental acoustic events, but, for the
moment, automatic processing of sounds by machines lags far behind.
Indeed, a substantial amount of research is still needed to have capable systems that robustly recognize a wide range of sound events in realistic audio streams drawn from everyday life~\cite{virtanen2018computational}.
%Everyday sounds in our environment bear a huge amount of information including contextual information about where we are and the physical events occurring nearby. 
%Humans have the ability to recognize many acoustic events happening in the environment with great detail.
%However, this is not a trivial task for machines that attempt to do it automatically.
%Indeed, a substantial amount of research is still needed to have systems able to robustly recognize a wide range of sound events in realistic everyday life audio streams~\cite{virtanen2018computational}.
% EF:we dont have evidence for to say the following:
%Indeed, it has been observed that current sound recognition systems still have a long way to reach near-human performance and thus to be able to robustly recognize sound events in realistic everyday life audio streams \cite{virtanen2018computational}. 


In recent years, the various editions of the IEEE AASP DCASE Challenge have provided scenarios for evaluating and benchmarking different computational methods for several sound recognition tasks using common publicly available datasets \cite{DCASE2017challenge}. 
The 2018 cycle of the DCASE challenge includes five tasks: \emph{Task 1)} Acoustic scene classification, \emph{Task 2)} General-purpose audio tagging of Freesound content with AudioSet labels, \emph{Task 3)} Bird audio detection, \emph{Task~4)} Large-scale weakly labeled semi-supervised sound event detection in domestic environments, and \emph{Task 5)} Monitoring of domestic activities based on multi-channel acoustics.
This paper describes the characteristics, dataset and baseline of Task 2 ``General-purpose audio tagging of Freesound content with AudioSet labels''.
%\footnote{\url{http://dcase.community/challenge2018/task-general-purpose-audio-tagging}}

The goal of Task 2 is to build an \emph{audio tagging system} that can categorize an audio clip as belonging to one of a set of 41 heterogeneous categories drawn from the AudioSet Ontology \cite{gemmeke2017audio} (e.g., musical instruments, human sounds, domestic sounds, animals, etc.).\footnote{The AudioSet Ontology in its entirety includes 632 audio categories.}

%NOTE: this short state of the art has been moved to section 4, I (frederic) think it makes more sense there to introduce the baseline. In any case this paper is not really about a state of the art in the field, so I think it is more important to describe the particularities of our task first
%Traditionally, audio tagging systems are built using feature engineering approaches where hand-crafted features are extracted from the audio signal and are input to a shallow classifier, e.g., SVM \cite{kumar2016audio}. 
%However, in recent years techniques based on learning representations from data have become popular---especially deep learning---where both feature extraction and classification are optimized jointly. 
%Some of the most successful techniques are CNNs \cite{cakir2016domestic}, deep unsupervised feature learning \cite{xu2017unsupervised} and CRNNs \cite{xu2017large}.
The motivation for this task comes from the large amount of user-generated audio content that is available on the web, which can be a resource of great potential for sound recognition related research.
%This task is motivated by the fact that a large amount of user-generated audio content is nowadays available on the web, which can be potentially useful for sound recognition related research.
%This task is motivated by the fact that a large amount of user-generated audio content is nowadays available on the web and its potential reuse is dimmed because of the content not always being well described and labeled. 
The use of such data for training audio tagging systems poses issues that have not been addressed in previous DCASE Challenge tasks. In particular, this task deals with user-generated audio clips retrieved from Freesound.\footnote{\url{https://freesound.org}}
These audio clips are very diverse in terms of acoustic content, recording techniques, clip duration, etc., and often feature incomplete and inconsistent user-provided labels.
To prepare the dataset for this task, some audio clips were manually labeled using the aforementioned subset of AudioSet categories, while a larger set of clips was automatically categorized on the basis of their existing user-provided labels (see Section~\ref{sec:dataset} for more details). As a result, the dataset annotations are of varying reliability. This task addresses two main challenges of (a) recognizing an increased number of diverse sound events, and (b) leveraging subsets of training data featuring annotations of varying reliability.

Submissions to this task will provide insight towards the development of broadly-applicable sound event classifiers.
Potential applications include automatic description of multimedia content, and acoustic monitoring applications.
The remainder of this paper is organized as follows. Section \ref{sec:challenge} provides more details about the task and its experimental setup.
Section \ref{sec:dataset} presents in detail the dataset prepared for the task, and Section \ref{sec:baseline} describes a baseline system.
Final remarks are given in Section \ref{sec:conclusion}.


==> S2_TaskSetupOLD.tex <==
% Task goal, including figure from DCASE web

%NOTE: I just thrown all the relevant information here. Need to re-phrase things and write all properly. Possibly move things to other sections as well.

%This task addresses the problem of general-purpose automatic audio tagging and poses two main challenges. The first one is to build models that can recognize an increased number of sound events of very diverse nature, including musical instruments, human sounds, domestic sounds, animals, etc. The second challenge consists of leveraging subsets of training data featuring annotations of varying reliability, as a reflection of the expensiveness of having high quality annotations. This task will provide insight towards the development of broadly-applicable sound event classifiers that consider an increased and diverse amount of categories. These models can be used, for example, in automatic description of multimedia or acoustic monitoring applications.

%(some of this could go to the intro section)

%The task consists of predicting the sound category to which every audio sample in the test set belongs to. A single label should be assigned to each file in the test set (i.e., single-tag tagging), although up to three labels can be predicted for each file as we evaluate with Mean Average Precision @ 3. The predictions are to be done at the audio sample level, i.e., no start/end timestamps for the events are required. The dataset for this task is split into a train set and a test set.

\begin{figure}[h]
  \centering
  \centerline{\includegraphics[width=\columnwidth]{task2_freesound_audio_tagging}}
  \caption{Overview of a single-tag tagging system.}
  \label{fig:task_diagram}
\end{figure}

%This task is hosted in Kaggle - a platform that hosts machine learning competitions with a well established community of participants. Hence, the resources associated to this task (datasets download, leaderboard and submission) will be provided by Kaggle. Please visit the Freesound General-Purpose Audio Tagging Challenge Kaggle competition page\footnote{\url{https://www.kaggle.com/c/freesound-audio-tagging}} for detailed information about how to participate and all other relevant aspects of the challenge. What follows in this page is a summary of the most important aspects of the challenge.

% Evaluation setup: train and test set (not in detail)
% \subsection{Train and test sets}
% The train set is meant to be for system development and includes ~9.5k samples unequally distributed among 41 categories. 
% The minimum number of audio samples per category in the train set is 94, and the maximum 300. 
% The duration of the audio samples ranges from 300ms to 30s due to the diversity of the sound categories and the preferences of Freesound users when recording sounds.

% The train set is composed of ~3.7k manually-verified annotations and ~5.8k non-verified annotations. 
% The quality of the non-verified annotations has been roughly estimated to be at least 65-70\% in each sound category. 
% A flag for each annotation is provided which indicates whether or not that annotation has been manually verified. Participants can use this information during the development of their systems.

% The test set is composed of ~1.6k manually-verified annotations with a similar category distribution than that of the train set. 
% These annotations are complemented with ~7.8k padding annotations which are also included in the test set but that won't be used for evaluating the systems.

% Submissions are evaluated according to the Mean Average Precision @ 3 (MAP@3).
% More details about the dataset are given in Sec.~\ref{sec:dataset}.

% Competition rules
%  the most relevant that attain to the data, mostly

% \subsection{Competition rules}
% A detailed description of the task rules can be found in the Freesound General-Purpose Audio Tagging Challenge Kaggle competition page\footnote{\url{https://www.kaggle.com/c/freesound-audio-tagging/rules}}. There was no monetary prize for the competition. This is a summary of the most important points:
% \begin{itemize}
%     \item Participants are allowed to use external data for system development, but external data can not be sourced from Freesound (including any of the original sound's metadata or other sounds in Freesound). This excludes judges award (see below).
%     \item Participants are not allowed to make subjective judgements of the evaluation data, nor to annotate it (this includes the use of statistics about the evaluation dataset in the decision making). The evaluation dataset cannot be used to train the submitted system.
%     \item The top-3 winning teams are required to publish their systems under an open-source license in order to be considered winners.
% \end{itemize}

% Submission aspects:
%   Max two per day
%   Public/private leaderboard
% A maximum of two submissions per team was allowed every day.
% NOTE: What to comment about the public/private leaderboard? Is it really relevant?

%  Competition timeline
% July 24, 2018 - Entry deadline. You must accept the competition rules before this date in order to compete.
% July 24, 2018 - Team Merger deadline. This is the last day participants may join or merge teams.
% July 31, 2018 - Final submission deadline.

% Judges Award??
\subsection{Judges' Award}
The goal of the Judges’ Award is to encourage contestants to use novel and problem-specific approaches which leverage knowledge of the audio domain. Another key factor is computational efficiency: we want to promote models that can fit within reasonable resource constraints, as opposed to very large models that may merely memorize a dataset and may not fit within typical deployment environments on mobile devices, for example. Details about the Judges Award rules and requirements are published in a Kaggle discussion\footnote{\url{https://www.kaggle.com/c/freesound-audio-tagging/discussion/59932}}

